ThinkSafe: Self-Generated Safety Alignment for Reasoning Models

Large reasoning models achieve strong performance through reinforcement learning but can suffer safety degradation. External teacher distillation can restore safety yet may compromise reasoning performance. We formalize safety realignment as a KL projection: the student's native filter-accepted distribution is uniquely KL-optimal, while teacher targets incur excess KL when they differ. Guided by this analysis, we propose ThinkSafe, which generates safety-alignment data from the frozen student without external teachers. Refusal steering elicits safety reasoning, and a safety guard filters the responses before offline fine-tuning. Our analysis bounds steering-induced target distortion and gives a sufficient condition for lower average target KL than teacher distillation. Experiments on DeepSeek-R1-Distill and Qwen3 show substantial safety improvements with competitive reasoning performance. On Qwen3-0.6B, ThinkSafe achieves better safety and comparable reasoning to GRPO in about one-seventh of the wall-clock time, including data generation. Code, models, and datasets are available at https://github.com/seanie12/ThinkSafe and https://huggingface.co/Seanie-lee/collections.

==> figures/main_radar.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/images/main_radar.pdf}
    \caption{Main results on our \textsc{ThinkSafe} shown as radar plots. Safety benchmarks are reported as $100 -$original scores ($\%$) for comparison, while "Avg. Reasoning" denotes the average performance over four reasoning benchmarks. (\textbf{Top}): results on the Qwen model family. (\textbf{Bottom}): results on the R1-distilled model series. Full quantitative results are provided in ~\Cref{tab:qwen_result,tab:deepseek_result}, respectively.}
    \label{fig:spyder}
    \vspace{-0.1in}
\end{figure*}

==> figures/pareto.tex <==
\begin{figure}
    % \centering
    \includegraphics[width=1.0\linewidth]{figures/images/pareto_v2.pdf}
    \vspace{-0.2in}
    \caption{Safety \& reasoning performance of the Qwen3 family.}
    \vspace{-0.3in}
    \label{fig:pareto}
\end{figure}

==> figures/perplexity.tex <==
% \begin{figure}
    
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/images/perplexity_comparison_v2.pdf}
%     \vspace{-0.2in}
%     \caption{Perplexity of generated safety dataset measured by the initial student models.}
%     \vspace{-0.2in}
%     \label{fig:perplexity}
% \end{figure}

==> figures/same_family.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\columnwidth]{figures/images/same_family_bar_v2.pdf}
%     \vspace{-0.1in}
%     \caption{Ratio of reasoning gain to safety gain for student models trained on data generated by teachers from the same model family.}
%     \vspace{-0.1in}
%     \label{fig:teacher-family}
% \end{figure}


==> tables/main_avg.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.15}
\caption{Safety, reasoning, and safety tax for DirectRefusal, SafeChain, and \textsc{ThinkSafe} across Qwen3 and R1-distilled models. $\overline{R}_\text{method}$ denotes the average pass@1 over four reasoning benchmarks, while $\overline{S}_\text{method}$ is the mean of HarmBench, StrongReject, WildJailbreak, and XSTest. Safety Tax is defined as $-\Delta R / |\Delta S|$, where $\Delta S = \overline{S}_\text{method} - \overline{S}_\text{init}$ and $\Delta R = \overline{R}_\text{method} - \overline{R}_\text{init}$; lower values indicate more favorable safety–reasoning trade-offs.
}
\label{tab:safety_tax_summary}

\resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
    
        \multicolumn{1}{c}{} &
        \multicolumn{3}{c}{Qwen3-0.6B} &
        \multicolumn{3}{c}{Qwen3-1.7B} &
        \multicolumn{3}{c}{Qwen3-4B}   &
        \multicolumn{3}{c}{Qwen3-8B}  &
        \multicolumn{3}{c}{R1D-Qwen-1.5B} &
        \multicolumn{3}{c}{R1D-Qwen-7B}   &
        \multicolumn{3}{c}{R1D-Llama-8B} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
        \cmidrule(lr){14-16}\cmidrule(lr){17-19}\cmidrule(lr){20-22}
        
        \multicolumn{1}{c}{Metric} &
        \multicolumn{1}{c}{\shortstack{Direct\\Refusal}} &
        \multicolumn{1}{c}{\shortstack{Safe\\Chain}} &
        \multicolumn{1}{c}{\shortstack{\textsc{Think}\\\textsc{Safe}}} &
        \multicolumn{1}{c}{\shortstack{Direct\\Refusal}} &
        \multicolumn{1}{c}{\shortstack{Safe\\Chain}} &
        \multicolumn{1}{c}{\shortstack{\textsc{Think}\\\textsc{Safe}}} &
        \multicolumn{1}{c}{\shortstack{Direct\\Refusal}} &
        \multicolumn{1}{c}{\shortstack{Safe\\Chain}} &
        \multicolumn{1}{c}{\shortstack{\textsc{Think}\\\textsc{Safe}}} &
        \multicolumn{1}{c}{\shortstack{Direct\\Refusal}} &
        \multicolumn{1}{c}{\shortstack{Safe\\Chain}} &
        \multicolumn{1}{c}{\shortstack{\textsc{Think}\\\textsc{Safe}}} &
        \multicolumn{1}{c}{\shortstack{Direct\\Refusal}} &
        \multicolumn{1}{c}{\shortstack{Safe\\Chain}} &
        \multicolumn{1}{c}{\shortstack{\textsc{Think}\\\textsc{Safe}}} &
        \multicolumn{1}{c}{\shortstack{Direct\\Refusal}} &
        \multicolumn{1}{c}{\shortstack{Safe\\Chain}} &
        \multicolumn{1}{c}{\shortstack{\textsc{Think}\\\textsc{Safe}}} &
        \multicolumn{1}{c}{\shortstack{Direct\\Refusal}} &
        \multicolumn{1}{c}{\shortstack{Safe\\Chain}} &
        \multicolumn{1}{c}{\shortstack{\textsc{Think}\\\textsc{Safe}}} \\
        \midrule
        
        $\overline{R}_\text{method}$ &
        40.62 & 39.06 & \textbf{44.17} &
        63.98 & 60.84 & \textbf{65.28} &
        74.28 & 73.12 & \textbf{77.13} &
        77.98 & 77.42 & \textbf{78.55} &
        52.87 & 51.01 & \textbf{54.38} &
        67.63 & 66.32 & \textbf{69.55} &
        62.94 & 60.25 & \textbf{65.77} \\
        
        $\overline{S}_\text{method}$ &
        43.89 & 45.03 & \textbf{34.17} &
        35.41 & 36.18 & \textbf{19.46} &
        26.11 & 29.80 & \textbf{6.45} &
        23.00 & 28.38 & \textbf{5.80} &
        51.93 & 47.29 & \textbf{45.78} &
        44.92 & 38.40 & \textbf{30.16} &
        28.91 & 36.38 & \textbf{21.08} \\
        
        Tax &
         1.00 &  1.60 & \textbf{0.03} &
         6.12 & -1.02 & \textbf{-0.06} &
         0.05 &  0.33 & \textbf{-0.23} &
        \textbf{-0.55} & -0.23 & -0.10 &
         0.53 &  0.40 & \textbf{-0.10} &
         1.30 &  0.23 & \textbf{-0.05} &
         0.47 &  0.18 &  \textbf{0.07} \\

    
    \bottomrule
    \end{tabular}
    \vspace{-0.15in}
}
\end{table*}

